Diversity Maximized Scheduling in RoadSide Units for Traffic Monitoring Applications

This paper develops an optimal data aggregation policy for learning-based traffic control systems based on imagery collected from Road Side Units (RSUs) under imperfect communications. Our focus is optimizing semantic information flow from RSUs to a nearby edge server or cloud-based processing units by maximizing data diversity based on the target machine learning application while taking into account heterogeneous channel conditions (e.g., delay, error rate) and constrained total transmission rate. As a proof-of-concept, we enforce fairness among class labels to increase data diversity for classification problems. The developed constrained optimization problem is non-convex. Hence it does not admit a closed-form solution, and the exhaustive search is NP-hard in the number of RSUs. To this end, we propose an approximate algorithm that applies a greedy interval-by-interval scheduling policy by selecting RSUs to transmit. We use coalition game formulation to maximize the overall added fairness by the selected RSUs in each transmission interval. Once, RSUs are selected, we employ a maximum uncertainty method to handpick data samples that contribute the most to the learning performance. Our method outperforms random selection, uniform selection, and pure network-based optimization methods (e.g., FedCS) in terms of the ultimate accuracy of the target learning application.

==> excluded_text.tex <==

\begin{comment}
    The objective function capture transmission cost, delay, and fairness. If the objective function is $f(\alpha)$, it is given by (\ref{eq:obj}), $f_1(\boldsymbol{\alpha})$ is the incurred delay in the network, $f_2(\boldsymbol{\alpha})$ is the throughput of the network and $f_3(\boldsymbol{\alpha})$ is the diversity that imposed fairness among collected class labels; the constrain here is the number of RSUs which can send packets in $T$ interval.

\begin{equation}
    &f(\boldsymbol{\alpha})= w_1f_1(\boldsymbol{\alpha})+ w_2f_2(\boldsymbol{\alpha})+ w_3f_3(\boldsymbol{\alpha})  \label{eq:obj}\\
\end{equation}
\begin{align}
\text { s.t. } \quad \sum_{i=1}^{\mathrm{N}} \alpha_i \leq \mathrm{M} \quad \forall i \in \mathrm{N}, \frac{\mathrm{M}}{\mathrm{N}}<1
\end{align}
This objective function is not convex and does not admit closed-form solutions, and solving numerically can be computationally expensive. Therefore, we are using an approximate rank-based method by selecting the top k RSUs out of $N$ in each interval that has a better condition to decrease average delay and increase average throughput. Moreover, for imposing fairness we use coalition game among RSUs to choose the best RSUs fairly. In coalition game players cooperate with each other by forming various sub-group called coalition. If $N$ be the number of players, $P$ shows the set of players $P=$ ($P_1, P_2,\dots,P_n$), $X_i$ shows the strategy of player $P_i$ in which for N-player there is $2^N$ possible coalition. $v(S)$ is characteristic function that represents total payoff can be gained by member of coalition $S$.

Let vector $\mathbf{x}=\left(x_1, \ldots, x_N\right), \mathbf{x} \in \mathbf{R}^N$ represent the amount of payoff that different members gained in a coalition. The coalition's payoff between the members must be efficient such that $\sum_{i=1}^N x_i=v(P)$ and also it needs to satisfy the individual rationality condition meaning that each player is getting paid better in a coalition than being on his own, $\forall i \in$ $P, x_i \geq v\left(P_i\right)$

First in (\ref{eq:qu}) we defined quality for each RSU in the network

\begin{equation}
   q_i(t)=w_1\zeta_i(t)+ w_2d_i(t) \label{eq:qu}
\end{equation}

for considering fairness we should impose it interval by interval so we add the fairness index to the quality

\begin{equation}
   q_i(t)+w_3J(n_1,n_2,\dots,n_n)
\end{equation}

then we have 
\begin{equation}
   v(S)=\sum_{i=1}^{\mathrm{N}} q_i(t)+w_3J(n_1,n_2,\dots,n_n)
\end{equation}

If RSU $n_i$ joins a coalition $S$, it may improve the fairness and quality in the network. This is called marginal contribution and is given by
$$
    v(S \cup\{n_i\})-v(S)
$$

in this approach, the Shapley value of player $P_i \in P$ is defined as the expected marginal contribution of player $i$ to the set of players who precede this player.
$$
\phi_i(v)= \frac{1}{N !}\sum_{S \subseteq \mathcal{N}/i}\right)\frac{|S| !(N-|S|-1) !}{N !}[v(S \cup\{n_i\})-v(S)]
$$

The Shapley value proposes a fair solution of the coalition game, since it is efficient and the summation of the marginal contribution of all players is equal to the characteristic function of the coalition $P, v(P)$. This approach gives us a simple and complet solution for choosing the best RSUs while we have fairness among them which increase diversity in the networks.

\end{comment}









We may need to use later.

First in (\ref{eq:qu}) we defined quality for each RSU in the network

\begin{equation}
   q_i(t)=w_1\zeta_i(t)+ w_2d_i(t) \label{eq:qu}
\end{equation}

for considering fairness we should impose it interval by interval so we add the fairness index to the quality

\begin{equation}
   q_i(t)+w_3J(n_1,n_2,\dots,n_n)
\end{equation}

then we have 
\begin{equation}
   v(S)=\sum_{i=1}^{\mathrm{N}} q_i(t)+w_3J(n_1,n_2,\dots,n_n)
\end{equation}

If RSU $n_i$ joins a coalition $S$, it may improve the fairness and quality in the network. This is called marginal contribution and is given by
$    v(S \cup\{n_i\})-v(S)
$

in this approach, the Shapley value of player $P_i \in P$ is defined as the expected marginal contribution of player $i$ to the set of players who precede this player.
$
\phi_i(v)= \frac{1}{N !}\sum_{S \subseteq \mathcal{N}/i}\right)\frac{|S| !(N-|S|-1) !}{N !}[v(S \cup\{n_i\})-v(S)]
$

The Shapley value proposes a fair solution of the coalition game, since it is efficient and the summation of the marginal contribution of all players is equal to the characteristic function of the coalition $P, v(P)$. This approach gives us a simple and complet solution for choosing the best RSUs while we have fairness among them which increase diversity in the networks.









========================================================
Excluded from the last version
=============================================================

%older version: keep for reference: Also, The next generation of wireless networks will enable many ML tools \cite{boroujeni2021novel} and applications to efficiently analyze data from edge devices for inference, autonomy, and decision-making purposes  \cite{lotfi2021performance}. Meanwhile, imperfect communication and the limited bandwidth of wireless networks can compromise the quality of learning models constructed using imagery collected from RSUs through wireless channels. Still, issues such as noise, delay, bit errors, .etc, are challenging for training an ML model \cite{chen2020joint}; as a result, due to the limited resources, delay limitations, and privacy concerns, edge devices cannot offload all collected datasets to a cloud server for training their ML models. This issue should be addressed \cite{zeng2019joint}. For example, Chen et al. \cite{chen2021distributed} shows that bit errors and delay in wireless networks can significantly affect the accuracy of distributed learning.
%So many works try to decrease the delay in the network \cite{zhang2022task}. Abad et al. \cite{abad2020hierarchical} optimized  resource allocation to reduce network delay.

%In \cite{guo2022distributed}, authors propose three optimization criteria, optimize the combination of delay and energy consumption, optimize delay under a constrain on energy consumption and optimize energy consumption with limitation on delay. This work minimize the linear combination of delay and energy consumption.
%older version: keep for references:  So many works try to decrease the delay in the network \cite{zhang2022task}. Abad et al. \cite{abad2020hierarchical} optimized  resource allocation to reduce network delay. In \cite{guo2022distributed}, authors propose three optimization criteria, optimize the combination of delay and energy consumption, optimize delay under a constrain on energy consumption and optimize energy consumption with limitation on delay. This work minimize the linear combination of delay and energy consumption. Konecny et al. \cite{konevcny2015federated} presented a novel algorithm for federated learning in which communication cost is minimized. In \cite{samarakoon2019distributed}, the problem of joint power and resource allocation for ultra-reliable low-latency communication in vehicular networks has been investigated. Several works show many challenges, such as rate maximization, delay minimization, interference management, improving energy efficiency and energy saving in wireless communications\cite{chinipardaz2022inter}\cite{liu2018ultra} \cite{samarakoon2018federated} \cite{sarlak2021approach} \cite{ashraf2018dynamic}.  Lotfi et al. \cite{lotfi2022semantic} proposed a novel semantic-aware collaborative deep reinforcement learning (CDRL) method that enables a group of heterogeneous untrained agents with semantically-linked DRL tasks to collaborate efficiently across a resource-constrained wireless cellular network.

%older version: keep for reference: Another issue is that we need fairness among packets when sending packet by RSUs because we have diversity in the network due to different position of RSUs and cameras; therefore, we should send all classes of data samples to a receiver; if we use just some special RSUs for our training, it will not give us good results. Our goal is to reach higher accuracy through more diverse samples from RSUs and achieve high accuracy under minimum cost, which can translate to the minimum number of transmissions. 
%Therefore, we assume that some RSUs send data for training an ML model, while RSUs have different delays, throughput, data, and bit errors; our goal is to choose RSUs with lower delay and higher throughput as diversity.
%To do this, as function is not convex and does not admit closed-form solutions, and solving numerically can be computationally expensive we proposed an greedy fairness which is empowered by coalition game, where we tried to minimize delay and maximize throughput and diversity in the network. 






%The main contributions of this work can be summarized as follows:
%1) We considered throughput, delay, and diversity effects in the network when we were training an ML model over a wireless link.
%2) We proposed a greedy method for fairness which use coalition game that chooses the best RSUs in terms of lower delay and higher throughput to increase an ML model's accuracy.
%3) We consider fairness among RSUs, which is critical when we have unbalanced datasets because we should have balanced datasets.
%The paper is organized as follows: We have a system model in the second section. In the third section, we have problem formulation. An objective function is defined in the fourth section, and in the fifth section, the simulation and evaluation of our proposed scheme compared to other methods are stated.



%The main contributions of this work can be summarized as follows:
%1) We considered throughput, delay, and diversity effects in the network when we were training an ML model over a wireless link.
%2) We proposed a greedy method for fairness which use coalition game that chooses the best RSUs in terms of lower delay and higher throughput to increase an ML model's accuracy.
%3) We consider fairness among RSUs, which is critical when we have unbalanced datasets because we should have balanced datasets.
%The paper is organized as follows: We have a system model in the second section. In the third section, we have problem formulation. An objective function is defined in the fourth section, and in the fifth section, the simulation and evaluation of our proposed scheme compared to other methods are stated.
%old ver keep for reference: Generally RSUs are an integral part of technology-driven traffic control infrastructure that collect imagery and use it for learning-based traffic monitoring and control tasks, such as object detection and sign recognition and we want to select a subset of RSUs in the network dynamically so as to send data to a center. On the other hand, the quality of learning can be affected by networking performance metrics. A higher throughput means collecting more samples that boosts the prediction power of ML algorithms. Lower delay is desired in real-time applications such as anomaly detection, etc. It is also known that diversity should be maximum when we send collected data to the center.
%older version: keep for ref: As we said, the delay is an essential issue in our approach; while others work on the physical layer to decrease delay, there is still a delay in the network, we want to regulate packet transmission under imperfect networking. Our approach tries to choose RSUs so as to decrease the average delay of packets in the network.

%older version: keep for ref: As the delay is a continuous random variable and it is clear that $d$ is a non-negative variable, we model queuing delay of each RSU as an exponential distribution \cite{ali2008measured} in which $d$ is a distributed random variable and have an exponential distribution with parameter $\lambda>0$:  

%\subsection{Transmission Delay}
%We also consider transmission delay for the packet in the network. Some packets cannot be sent on the first try, so we should consider a retransmission delay because it adds delay to the network. The transmission delay can be calculated like (\ref{eq:L}), where $L$ is the packet's length.

% \begin{equation}  
% D_t_r=\frac{L}{b}\label{eq}  \label{eq:L}
% \end{equation}
%In the channel when the retransmission increases, the packet has more delay and more probability for a drop. We model the retransmission delay as a geometric distribution; consequently, (\ref{eq:geo}) is the probability of transmission of packets in which $ \beta_i $ is the packet error rate for the RSU $n_i$.



%consequently, it should be maximized when we train a model. On the other hand, in the network, fairness is used to assign fairer networking resources among nodes to maximize utility in the network.
%Furthermore, we have a fixed and equal bandwidth for each RSU and a limited bandwidth in the receiver. Consequently, there is a trade-off between efficiency and fairness because more fairness can result in higher delay and lower throughput in the network. We enforce fairness among collected class labels because RSUs have different class labels with attention to the sensors, cameras, and environment. First, we defined a fairness measure to calculate fairness in the network. Let $x$ be our rate allocation vector with $R$ non-negative elements. $f(x)$ is our fairness index which is mapping from $x$ to a real number, e.i., $f: \mathbb{R}_{+}^n \rightarrow \mathbb{R}$, for all integer $R \geq 1$. Our fairness index is given by (\ref{eq:fair}) \cite{lan2010axiomatic}



%As we know, the diversity of data samples significantly impacts learning quality; consequently, it should be maximized when we train a model. On the other hand, in the network, fairness is used to assign fairer networking resources among nodes to maximize utility in the network.
%Furthermore, we have a fixed and equal bandwidth for each RSU and a limited bandwidth in the receiver. Consequently, there is a trade-off between efficiency and fairness because more fairness can result in higher delay and lower throughput in the network. We enforce fairness among collected class labels because RSUs have different class labels with attention to the sensors, cameras, and environment. First, we defined a fairness measure to calculate fairness in the network. Let $x$ be our rate allocation vector with $R$ non-negative elements. $f(x)$ is our fairness index which is mapping from $x$ to a real number, e.i., $f: \mathbb{R}_{+}^n \rightarrow \mathbb{R}$, for all integer $R \geq 1$. Our fairness index is given by (\ref{eq:fair}) \cite{lan2010axiomatic}


\begin{comment} 
%keep for later
sent by RSU $n_i$ and is successfully received by the processing unit. Then, we will have the following 

$zz$; consequently, we can define diversity for each RSU in (\ref{eq:fiar2})


We considered two extreme cases for data diversity; in the first extreme case, RSUs are equivalent in terms of a different class. 

\begin{align}
c_i^j=c_k^j=k \nonumber
\end{align}
\begin{align}
c_R^j=\sum_{i=1}^{\mathrm{N}} c_i^j \zeta_i=c_i^j \sum_{i=1}^{\mathrm{N}} \zeta_i=c_i^j\left(\frac{\mathrm{M}}{\mathrm{N}}\right) \label{eq:fair4}
\end{align}

In (\ref{eq:fair4}), we can see that diversity is independent of choosing RSU because all RSUs have the same class. In another extreme case, each $\mathrm{RSU}$ has only one class $(\mathrm{N}=C)$

\begin{align}
c_i^j=\left[c_i^1, c_i^2, \cdots, c_i^C\right]=\left[0,0, \cdots, c_i^j, 0\right] \nonumber
\end{align}
\begin{align}
c_R^j=\sum_{i=1}^{\mathrm{N}} c_i^j \zeta_i=c_i^j \zeta_i=k \zeta_i \nonumber
\end{align}

\begin{align}
\nonumber
J\left(c_R^1, c_R^2, \cdots, c_R^C\right)=J\left(k \zeta_1, k \zeta_2, \cdots, k \zeta_{\mathrm{N}}\right)\\
=k J\left(\zeta_1, \zeta_2, \cdots, \zeta_{\mathrm{N}}\right) \label{eq:fair5}
\end{align}

In (\ref{eq:fair5}), diversity is dependent on throughput; consequently, sending data from all RSUs to train data with all classes is essential.


\end{comment}

 
%propose an approximate rank-based method by selecting the top k RSUs out of $N$ in each interval that has a better condition to decrease average delay and increase average throughput. Moreover, for imposing fairness we use coalition game among RSUs to choose the best RSUs fairly. 


%In this formulation, RSUs are considered game players that cooperate with each other by forming various sub-group called coalitions. Each player decides whether or not to join a coalition. 
%If $N$ be the number of players, $P$ shows the set of players $P=$ ($P_1, P_2,\dots,P_n$), $X_i$ shows the strategy of player $P_i$ in which for N-player there is $2^N$ possible coalition. $v(S)$ is characteristic function that represents total payoff can be gained by member of coalition $S$.
%Let vector $\mathbf{x}=\left(x_1, \ldots, x_N\right), \mathbf{x} \in \mathbf{R}^N$ represent the amount of payoff that different members gained in a coalition. The coalition's payoff between the members must be efficient such that $\sum_{i=1}^N x_i=v(P)$ and also it needs to satisfy the individual rationality condition meaning that each player is getting paid better in a coalition than being on his own, $\forall i \in$ $P, x_i \geq v\left(P_i\right)$

% test We evaluated some scenarios for the simulation:
% 1) Optimized without fairness: here, in each interval, we choose 5 RSUs which are the best in terms of throughput and delay for sending packets. Also, we do not have fairness; for example, one RSU sends a packet in 9-interval, while another sends a packet in just 1-interval.
% 2) Optimize using fairness: in each interval, we choose 5 RSUs which are the best in terms of throughput and delay, and also consider fairness among them.
% 3) Uniform rate: here, we are just considering fairness, and we do not consider throughput and delay in the network; consequently, in each interval, 10 RSUs send packets.
% 4) Random rate: here, we randomly choose 5 RSUs in each interval for sending a packet. We do not consider throughput, delay, and fairness in the network; we run it ten times and consider the average throughput.
% 4) FedCS: this method asks random clients for their resource information; then, the operator refers to estimate the time required for the Distribution and Scheduled Update and Upload steps and to determine which clients go to these steps \cite{nishio2019client}. Here we assume that we know the delay; as a result, the method considers the best RSU in terms of delay.

%In Fig.4 and Fig.5, we analyzed our approach with a balanced dataset. When we have a balanced data set, optimization without fairness has the highest accuracy because we have better throughput. as we can see, high throughput guarantees high accuracy.  


\begin{comment}
Keep for later use!

\begin{table}[htbp]
\caption{Jain's Fairness Index}
\begin{center}
\begin{tabular}{|c|c|}
\hline
\cline{1-2} 
\textbf{\textit{Methods}}& \textbf{\textit{Fairness}} \\
    \hline
    Optimized without Fairness & 0.749 \\
    \hline
    Optimized using Fairness & 0.933 \\
    \hline
    Uniform Rate & 1 \\
    \hline
    Random Rate & 0.876 \\
    \hline
    FedCS & 0.766 \\
    \hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}
\end{comment}


%In Fig.6 and Fig.7, we analyzed our approach with the unbalanced dataset. For simulation, we consider two classes for each RSU; we can see optimization using fairness has the best performance compared to other approaches because the model is trained with fair data, while in optimization without fairness, some classes are missed. Although the uniform rate has lower throughput than optimization without fairness, it performs better than optimization without fairness here. These results show that considering fairness is very important when we have an unbalanced dataset.  



%CL using RSUs which collect data and send them to center for train an ML model. As we know, there are some issues when using CL over a wireless network, affecting the trained model's accuracy. Consequently, we tried to address these issues via an greedy method using coalition game. Moreover, we considered diversity among data saples in RSUs and maxithe mize it; as a result, we achieved high accuracy when training our model. Our approach shows the importance of choosing RSUs in the network while conditions on RSUs are different; also, diversity plays an important role, so it should be considered when we choose RSUs in the network


